Analysis of SiW-ECAL technological prototype beam test with electron beam

The beam test for the SiW-ECAL technological prototype was conducted using electron beam in June-July 2019 at DESY test beam facility in Hamburg, Germany. In the beam test, there were two main programs: MIP program (without tungsten) and shower program (with tungsten). The purposes of the MIP program are energy calibration, pedestal uniformity/stability assessment, TDC operation test, and retrigger verification. On the other hand, the shower program aims to evaluate energy resolution through beam energy measurement. In addition, several operation tests with FEV13 were also conducted such as individual threshold control and auto gain mode. This article presents the performance of the technological prototype of SiW-ECAL, mainly focusing on the version of FEV13-Jp.

==> section/5_Summary.tex <==
% !TEX root = ../CHEF2019_Proc.tex

\section{Summary and prospects}

